Balancing Privacy Protection and Interpretability in Federated Learning

Federated learning (FL) aims to collaboratively train the global model in a distributed manner by sharing the model parameters from local clients to a central server, thereby potentially protecting users' private information. Nevertheless, recent studies have illustrated that FL still suffers from information leakage as adversaries try to recover the training data by analyzing shared parameters from local clients. To deal with this issue, differential privacy (DP) is adopted to add noise to the gradients of local models before aggregation. It, however, results in the poor performance of gradient-based interpretability methods, since some weights capturing the salient region in feature map will be perturbed. To overcome this problem, we propose a simple yet effective adaptive differential privacy (ADP) mechanism that selectively adds noisy perturbations to the gradients of client models in FL. We also theoretically analyze the impact of gradient perturbation on the model interpretability. Finally, extensive experiments on both IID and Non-IID data demonstrate that the proposed ADP can achieve a good trade-off between privacy and interpretability in FL.

==> back_preliminary.tex <==
\section{Preliminaries}
\subsection{Grad-CAM}
As a typical gradient-based intrepretability approach, Gradient-weighted Class Activation Mapping (Grad-CAM)~\cite{Selvaraju2017} aims to provide visual explanations on the tasks of computer vision using the gradients to capture the salient regions of feature map in the last convolutional layer of deep neural networks.

In this paper, we use image classification as a running example to introduce the basic idea of Grad-CAM. Let $y^c$ be the prediction score (before softmax activation) of class $c$ and $A^k$ denote the feature map of a certain (e.g., last) convolutional layer. The gradient of $y^c$ with respect to $A^k$ is denoted by $\frac{\partial y^c}{\partial A^k}$. Then we can leverage the gradients via back-propagation to get the following neuron importance weights. 
\begin{equation}
\begin{aligned}
    \alpha_k^c = \frac{1}{Z}\sum_i \sum_j \frac{\partial y^c}{\partial A_{ij}^k},
\end{aligned}
\end{equation}
where $k$ represents the $k$-th channel of feature map $A$, $Z$ represents the product of the width and height of the feature map, $\alpha_k^c$ denotes the importance of feature map $k$ for class $c$, and $A_{ij}^k$ is the data of feature map $A$ at the coordinate $(i, j)$ in channel $k$.

Next, we can use weighed sum of forward activation maps and the ReLU activation function to obtain the localization map Grad-CAM $L_{Grad-CAM}^c$ as follows.
\begin{equation}
\begin{aligned}
   L_{Grad-CAM}^c = ReLU\Big(\sum_k \alpha_k^c A^k\Big).
\end{aligned}
\end{equation}
Note that, ReLU is used to remain features that have a positive impact on class $c$. 

% \textcolor{red}{Gradient-weighted Class Activation Mapping (Grad-CAM), a high-resolution class-discriminative localization technique that creates visual explanations from any CNN-based network, leverages gradient information flowing into the last convolutional layer of the CNN to determine the significance of each neuron for the decision of interest~\cite{Selvaraju2017}.}

% We utilize the image classification task in this paper as an example to demonstrate the computational process of GradCAM. The network prediction $y^c$ (before softmax activation) of class $c$ and feature maps $A^k$ of a convolutional layer are first obtained by forward propagation of the neural network. The activation map of the last convolutional layer is frequently used due to its rich high-level semantic information and detailed spatial information. The gradient of $y^c$ with respect to $A^k$ is computed as $\frac{\partial y^c}{\partial A^k}$. Then by back-propagation, \textcolor{red}{the gradients are global-average-pooled to obtain the neuron importance weights}:
% \begin{equation}
% \begin{aligned}
%     \alpha_k^c = \frac{1}{Z}\sum_i \sum_j \frac{\partial y^c}{\partial A_{ij}^k},
% \end{aligned}
% \end{equation}
% where $k$ represents the $k$-th channel of feature map $A$, $Z$ represents the product of the width and height of the feature map, $\alpha_k^c$ denotes the importance of feature map $k$ for class $c$, and $A_{ij}^k$ is the data of feature map $A$ at the coordinate $(i, j)$ in channel $k$.



\subsection{Federated Learning}
Federated learning (FL) is an emerging privacy-preserving technique that collaboratively trains a global model without sharing data with each client~\cite{}. Specifically, for each training round, the selected clients upload the model parameters (weights) to a central server. Then, the server aggregates the shared parameters for a global model, and broadcasts the updated global model to the clients. This process will be repeated until the global model converges. 

\shao{Please briefly introduce FL}

% \textcolor{red}{Federated learning is a distributed learning paradigm in which multiple clients participate in collaborative training without centralizing datasets}~\cite{McMahan2017}. The loss function of FL can be mathematically described as:
% \begin{equation}
% \begin{aligned}
%     \mathop{\min}_{w\in R} f(w) \qquad    {\rm where}  \qquad f(w)=\frac{1}{n}\sum_{i=1}^n f_i(w),
% \end{aligned}
% \end{equation}
% where $f_i(w) $ is a local loss function for one client, and $f(w)$ represents the \textcolor{red}{global loss function over all clients}.

Suppose a FL system contains $1$ server and $K$ clients, and \textcolor{red}{the index set of local private data points for client $k$} is denoted as $P_k$, where $n_k = |P_k|$. Then equation (3) can be further expressed as:
\begin{equation}
\begin{aligned}
     f(w) = \sum_{k=1}^K \frac{n_k}{n}F_k(w) \quad  {\rm where}  \quad F_k(w) = \frac{1}{n_k}\sum_{i \in P_k} f_i(w).
\end{aligned}
\end{equation}

Each communication round typically involves the selection of a $C$-fraction of clients, where \textcolor{red}{$C=1$ corresponds to full-batch gradient descent, which is refered as FedSGD}. After receiving the global parameter $w_t$ from the server, the selected clients train the model using their local data and calculate the gradient $g_k = \nabla F_k(w_t)$ before uploading it back to the server for aggregation and updating $w_{t+1} \leftarrow w_t - \eta \sum_{k=1}^K \frac{n_k}{n}g_k$, according to the learning rate $\eta$. If numerous iterations are carried out on the client's local data before uploading the gradient to the server, i.e., $w^k \leftarrow w^k - \eta \nabla F_k(w^k)$, then this approach is known as FedAvg, which is particularly popular because not only can it \textcolor{red}{be applied to large-scale data, but its performance is comparable to that of many other FL-based algorithms}.


\subsection{Differential privacy}
As a privacy-preserving method, differential privacy (DP) attempts to maximize the useful information retrieved from a database while minimizing the expenditure of privacy resources~\cite{Adnan2022}. Briefly, DP is the preservation of the privacy of every individual in the dataset, requiring that each single element in the dataset has a limited impact on the output and that no private information about the individual can be deduced from the query results.
Mathematically, ($\epsilon$, $\delta$)-DP~\cite{Dwork2014} can be expressed as:
\begin{equation}
\begin{aligned}
      {\rm Pr}\big[M(D_i)\in S \big] \leq e^\epsilon \, {\rm Pr}\big[M(D^{'}_i)\in S \big] + \delta.
\end{aligned}
\end{equation}
where $D_i$ and $D^{'}_i$ are \textcolor{red}{two adjacent datasets in a database}, only one piece of data differs between them. $\epsilon$ denotes the upper bound of the output probability that can be changed by adding or removing a record in the dataset, i.e., the privacy protection standard. The smaller the value, the stricter the standard, hence it is also known as privacy budget. Additionally, $\delta$ is typically set to a small constant, which denotes \textcolor{red}{the event that the probability ratio for two adjacent datasets $D_i$ and $D^{'}_i$ not being constrained by $e^ \epsilon$ after a privacy-preserving mechanism} has been applied~\cite{Wei2020}. 

Differential privacy applied to federated learning is usually achieved by clipping the gradient and adding a moderate amount of Gaussian noise. \textcolor{red}{To ensure that the Gaussian noise distribution $n \sim N(0, \sigma^2)$ satisfies ($\epsilon$, $\delta$)-DP, it is necessary to choose noise scale $\sigma \geq c\Delta s/ \epsilon$, and the constant $c \geq \sqrt{2 {\rm ln}(1.25/\delta)}$ for $\epsilon \in (0, 1)$}. Additionally, $\Delta s$ represents \textcolor{red}{the sensitivity of a real-valued function} $s$ given by $\Delta s = {\rm max}_{D_i, D^{'}_i}\big|\big|s(D_i)-s(D^{'}_i)\big|\big|$.


